Interpretable Super-Resolution via a Learned Time-Series Representation

We develop an interpretable and learnable Wigner-Ville distribution that produces a super-resolved quadratic signal representation for time-series analysis. Our approach has two main hallmarks. First, it interpolates between known time-frequency representations (TFRs) in that it can reach super-resolution with increased time and frequency resolution beyond what the Heisenberg uncertainty principle prescribes and thus beyond commonly employed TFRs, Second, it is interpretable thanks to an explicit low-dimensional and physical parameterization of the Wigner-Ville distribution. We demonstrate that our approach is able to learn highly adapted TFRs and is ready and able to tackle various large-scale classification tasks, where we reach state-of-the-art performance compared to baseline and learned TFRs.

==> datasets.tex <==
\subsection{Dyni Odontocete Click Classification, 10 species}

Challenge context
This challenge is linked to the largest international bioacoustical observatory, that is currently running in Caribbeans: 20 recordings stations are deployed from Bahamas to Venezuela during 1 year (EU project CARIMAM), at high sampling rate ( 512 kHz SR). It results into 60 To of recordings, that will be processed to assess the biodiversity of all this area by DYNI CNRS team (PI H. Glotin). Thus challenge aims to classify clicks emitted by biosonar of 10 cetaceans species (odontocetes). The recordings of the clicks are from a post-processed subset of DCLDE 2018 challenge ( 9 species, \url{http://sabiod.org/DCLDE }), plus recordings of Cachalot (Physteter macrocephalus, Pm) done from ASV Sphyrna (\url{http://sphyrna-odyssey.com}) near Toulon, France. Each input signal is 8192 bins, at a sampling rate of 200 kHz. They each includes a click centered in the middle of the window in the case of the test set. The clicks in the training set are in various positions and background noises.

Challenge goals
The goal is to classify each click according to the corresponding emitting species. The 10 species are : (0) Gg: Grampus griseus- Risso's dolphin (1) Gma: Globicephala macrorhynchus- Short-finned pilot whale (2) La: Lagenorhynchus acutus- Atlantic white-sided dolphin (3) Mb: Mesoplodon bidens- Sowerby's beaked whale (4) Me: Mesoplodon europaeus- Gervais beaked whale (5) Pm: Physeter macrocephalus - Sperm whale (6) Ssp: Stenella sp.Stenellid dolphin (7) UDA: Delphinid type A - a group of dolphins (species not yet determined) (8) UDB: Delphinid type B - another group of dolphins (species not yet determined) (9) Zc: Ziphius cavirostris- Cuvier's beaked whale The metric is the MAP.

Data description
The recordings are from various subsea acoustic stations or autonomous surface vehicles (ASV). A part (9 classes) has been provided by the Scripps Institution of Oceanography for the 8th DCLDE Workshop. They consist of acoustic recordings from multiple deployments of high-frequency acoustic recording packages (Wiggins and Hildebrand, 2007) deployed in the Western North Atlantic (US EEZ) and Gulf of Mexico. It has a 100 kHz of bandwidth (200 kHz sample rate). Data were selected to cover multiple seasons and locations while providing high species diversity and call counts as described in http://sabiod.org/DCLDE/challenge.html#highFreqData . The initial data set is 3 To and weak labeled. DYNI LIS TOULON (Ferrari Glotin 2019) filtered their labels by several detector and clustering, yielding to 90 000 samples (6 Go). Another part (1 class) is from Dyni team recording in Mediterranean sea, from ASV Sphyna, at 384 kHz Fe, downsampled at 200 kHz Fe. It contains clicks from Cachalot monitored in 3D by passive acoustics ( Poupard et al ICASSP 2019, \url{http://sphyrna-odyssey.com}). In sum, it yields around 11312 samples per class in the train set, and 2096 samples per class in the test set. The public test set if formed of 10% of the test set, the private being the resting 90%. It is thus as a balanced classes classification problem.


\subsection{GTZAN}


\subsection{Freefield1010}
In order to maximise the potential usefulness of the dataset, before preparationwe considered the following design criteria:Content:Firstly we aimed to reflect the content that a general audio archivemight collect.  Given the range of archive policies, from crowdsourced to strictlycurated, we opted for a middle way, by using Freesound contributions but onlythose  under  thefield-recordingtag.   Initial  inspection  of  the  various  tags  inFreesound  determined  that  this  tag  was  mostly  free  of  interpretation  issues,unlike for exampleambiencewhich Freesound users often use for ambient fieldrecordings but also for synthesised atmospheric soundtrack sounds. On the otherhand, we decided not to manually curate the collection to a specific definition of“field recording”, in part because such curation is difficult to apply to materialfrom unknown third parties, and also because audio archive collections are rarelyso narrowly construed.Licensing:Freesound contains material under various licences.  Most com-mon are the Creative Commons CC-BY licence and the “CC0” public domaindedication,  though  there  is  a  small  proportion  of  older  material  under  otherlicences such as Creative Commons “sampling” licences which are not compat-ible with CC-BY. We wished to be able to apply a single open licence to theoverall dataset, so we restricted ourselves to CC-BY and CC0 material, whichmeans the overall dataset can be published under CC-BY. We also needed torespect the attribution requirements in the CC-BY source material, which weimplemented by ensuring we stored the author metadata with each file as wellas a URL to link back to the original source.Size and duration:We aimed to produce a dataset of manageable storagesize, for ease of redistribution, yet suitably diverse.  We also wished to producesound excerpts of a standard and relatively short duration, so that they couldbe used in listening tests without risking listener fatigue, and so that automatictests  could  run  efficiently.   These  motivations  led  us  to  settle  on  a  fixed  ten-second duration for each excerpt.File formats:We also aimed to use a standardised file format.  Freesoundallows  users  to  upload  sounds  of  any  sample  rate,  any  number  of  channels,and  in  various  file  formats  (uncompressed  and  lossy-compressed).   We  chosenot to use audio coming from lossy compressed file formats, in case of artifactsintroduced by the codecs.  We also chose to convert all downloaded sounds tostandard CD-quality mono WAV files.  We considered standardising on 24-bitand/or 96 kHz as recommended in the IASA “TC04” archiving standard [IASATechnical Committee, 2009].  However, in our experience 16-bit PCM has beenmore  widely  compatible  than  24-bit  PCM:  the  latter  is  not  well  handled  bysome older versions of Matlab and some Python audio libraries, although thissituation  is  improving.   Also  the  majority  of  the  original  downloaded  audiowas in 44.1 kHz.  We therefore settled on 16-bit 44.1 kHz.  In the crowdsourcedFreesound archive, amplitude levels are uncontrolled, which may be problematicfor listening tests.  We therefore chose to amplitude-normalise each excerpt inour dataset.

Dataset partitioning:In data mining and machine-learning experiments,it is useful to have a dataset partitioned into separate subsets—e.g. one for train-ing and another for testing [Witten and Frank, 2005, Chapter 5].  To facilitatethis we chose to partition our data into ten equally-sized subsets.  Partitioningcan be purely random or can bestratified: for example, if the data was intendedfor an experiment detecting the presence of geotags, then the partitions couldbe arranged such that each partition had an equal mix of geotagged and non-geotagged data [Witten and Frank, 2005, Chapter 5].  However, our dataset isintended  for  various  purposes  and  not  for  a  single  specific  experiment,  so  weopted for the simple random partitioning.  Researchers can choose to use thesesubsets for comparability with others, or to perform their own partitioning.

==> intro.tex <==




